Change Points via Probabilistically Pruned Objectives

The concept of homogeneity plays a critical role in statistics, both in its applications as well as its theory. Change point analysis is a statistical tool that aims to attain homogeneity within time series data. This is accomplished through partitioning the time series into a number of contiguous homogeneous segments. The applications of such techniques range from identifying chromosome alterations to solar flare detection. In this manuscript we present a general purpose search algorithm called cp3o that can be used to identify change points in multivariate time series. This new search procedure can be applied with a large class of goodness of fit measures. Additionally, a reduction in the computational time needed to identify change points is accomplish by means of probabilistic pruning. With mild assumptions about the goodness of fit measure this new search algorithm is shown to generate consistent estimates for both the number of change points and their locations, even when the number of change points increases with the time series length. A change point algorithm that incorporates the cp3o search algorithm and E-Statistics, e-cp3o, is also presented. The only distributional assumption that the e-cp3o procedure makes is that the absolute $\alpha$th moment exists, for some $\alpha\in(0,2)$. Due to this mild restriction, the e-cp3o procedure can be applied to a majority of change point problems. Furthermore, even with such a mild restriction, the e-cp3o procedure has the ability to detect any type of distributional change within a time series. Simulation studies are used to compare the e-cp3o procedure to other parametric and nonparametric change point procedures, we highlight applications of e-cp3o to climate and financial datasets.

==> tables/blankTable.tex <==
\begin{table}[H]
\begin{tabular}{lccc}
\hline
\multicolumn{1}{c}{} & \multicolumn{1}{c}{PELT} & \multicolumn{1}{c}{KCPA} & \multicolumn{1}{c}{EMACP} \\ \hline
\multicolumn{4}{c}{T=400}                                                                              \\ \hline
Time                                 &                          &                          &                           \\
\# of cps                            &                          &                          &                           \\
Rand                                 &                          &                          &                           \\
$\text{Rand}_\bigstar$               &                          &                          &                           \\ \hline
\multicolumn{4}{c}{T=800}                                                                                              \\ \hline
Time                                 &                          &                          &                           \\
\# of cps                            &                          &                          &                           \\
Rand                                 &                          &                          &                           \\
$\text{Rand}_\bigstar$               &                          &                          &                           \\ \hline
\multicolumn{4}{c}{T=1600}                                                                                             \\ \hline
Time                                 &                          &                          &                           \\
\# of cps                            &                          &                          &                           \\
Rand                                 &                          &                          &                           \\
$\text{Rand}_\bigstar$               &                          &                          &                           \\ \hline
\end{tabular}
\caption{\label{normSim}
Results of the first univariate simulation with different time series lengths.
}
\end{table}

==> tables/tailNorm.tex <==
\begin{table}[H]
\begin{tabular}{lccc}
\hline
\multicolumn{1}{c}{} & \multicolumn{1}{c}{PELT} & \multicolumn{1}{c}{KCPA} & \multicolumn{1}{c}{EMACP}                 \\ \hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{T=400}                                                                       \\ \cline{2-4}

Time                                 &       $0.004_{5\e{-5}}$              &         $16.527_{3\e{-3}}$           &       $17.545_{5\e{-2}}$              \\
\# of cps                            &      $13.610_{0.5}$              &         $ 2.750_{0.3}$           &        $2.110_{0.1}$              \\
Rand                                 &       $0.654_{6\e{-3}}$              &          $0.695_{10^{-2}}$           &        $0.763_{10^{-2}}$              \\
$\text{Rand}_\bigstar$               &        \textemdash       &        \textemdash       &        $0.868_{10^{-2}}$              \\ \hline
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{T=800}                                                                       \\ \cline{2-4}
% 
% Time                                 &       0.006              &        262.535           &      115.331              \\
% \# of cps                            &      17.730              &          8.880           &        1.960              \\
% Rand                                 &       0.669              &          0.800           &        0.740              \\
% $\text{Rand}_\bigstar$               &        \textemdash       &        \textemdash       &        0.862              \\ \hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{T=1600}                                                                      \\ \cline{2-4}

Time                                 &       $0.011_{1\e{-4}}$              &       $4273.679_{6\e{-2}}$           &      $504.684_{3.6}$              \\
\# of cps                            &      $25.360_{0.6}$              &          $9.000_{0.0}$           &        $2.430_{8\e{-2}}$              \\
Rand                                 &       $0.673_{6\e{-3}}$              &          $0.849_{4\e{-3}}$           &        $0.754_{9\e{-3}}$              \\
$\text{Rand}_\bigstar$               &        \textemdash       &        \textemdash       &        $0.813_{10^{-2}}$              \\ \hline
\end{tabular}
\caption{\label{table:tailSim}
Results of the second univariate simulation with different time series lengths. The subscripts indicate the standard errors for each value.
}
\end{table}

==> tables/tailSimTable.tex <==
\begin{table}[H]
\begin{tabular}{lccc}
\hline
\multicolumn{1}{c}{} & \multicolumn{1}{c}{PELT} & \multicolumn{1}{c}{KCPA} & \multicolumn{1}{c}{EMACP}                 \\ \hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{T=400}                                                                       \\ \cline{2-4}

Time                                 &       0.004              &         16.525           &       17.698              \\
\# of cps                            &      15.000              &          0.240           &        1.170              \\
Rand                                 &       0.699              &          0.504           &        0.631              \\
$\text{Rand}_\bigstar$               &        \textemdash       &        \textemdash       &        0.743              \\ \hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{T=800}                                                                       \\ \cline{2-4}

Time                                 &       0.006              &        262.885           &       91.448              \\
\# of cps                            &      19.480              &          2.790           &        1.140              \\
Rand                                 &       0.719              &          0.588           &        0.631              \\
$\text{Rand}_\bigstar$               &        \textemdash       &        \textemdash       &        0.708              \\ \hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{T=1600}                                                                      \\ \cline{2-4}

Time                                 &       0.012              &       4272.553           &      292.444              \\
\# of cps                            &      26.920              &          8.820           &        1.390              \\
Rand                                 &       0.730              &          0.760           &        0.654              \\
$\text{Rand}_\bigstar$               &        \textemdash       &        \textemdash       &        0.724              \\ \hline
\end{tabular}
\caption{\label{table:tailSim}
Results of the second univariate simulation with different time series lengths.
}
\end{table}










